An Approach to Build Zero-Shot Slot-Filling System for Industry-Grade Conversational Assistants

We present an approach to build Large Language Model (LLM) based slot-filling system to perform Dialogue State Tracking in conversational assistants serving across a wide variety of industry-grade applications. Key requirements of this system include: 1) usage of smaller-sized models to meet low latency requirements and to enable convenient and cost-effective cloud and customer premise deployments, and 2) zero-shot capabilities to serve across a wide variety of domains, slot types and conversational scenarios. We adopt a fine-tuning approach where a pre-trained LLM is fine-tuned into a slot-filling model using task specific data. The fine-tuning data is prepared carefully to cover a wide variety of slot-filling task scenarios that the model is expected to face across various domains. We give details of the data preparation and model building process. We also give a detailed analysis of the results of our experimental evaluations. Results show that our prescribed approach for slot-filling model building has resulted in 6.9% relative improvement of F1 metric over the best baseline on a realistic benchmark, while at the same time reducing the latency by 57%. More over, the data we prepared has helped improve F1 on an average by 4.2% relative across various slot-types.

==> sections/introduction-v0.tex <==
\section{Introduction - v0}

\begin{itemize}
    \item Chat bots are used by several organizations to serve both their employees and their customers. 
    \item Slot filling model is a core component of chat bots.
    \item Massive LMs like ChatGPT are very good at slot filling but they can't be easily used because of slow response time, prohibitive inference costs, data privacy concerns etc.
    \item Thus, smaller models (around 10B parameters) would be ideal as they can be easy to train and deploy both on cloud or on premises. It is easy to achieve sub 1 second response time.
    \item Small models aren't as good as the large ones out of the box for slot filling.
    \item Small models can be fine-tuned on publicly available dialogue state tracking datasets. Our experiments show that such models will not be robust and will be limited to a few types of slots. This is to with the limitations of the datasets themselves.
    \item Slot filling models deployed in the real world need to handle various different types of slots/entities/scenarios such as - categorical slots, name splitting, address parsing, relation extraction, multiple slots revealed in a single user turn, conversation and slot descriptions containing markdown, HTML, etc., modification of slot values as the conversation progresses, IDs like email ID, customer ID, employee ID, government ID numbers, etc 
    \item It is essential that a modern slot filling model have zero-shot capabilities. It should work well on domains that are not seem during training. During inference, it should rely only on easily available information - such as the natural language description of slots.
    \item Our contributions in this paper are as follows:
    \begin{itemize}
        \item We construct slot filling benchmarks that closely resemble real world scenarios in which slot filling models have to operate.
        \item We train and evaluate models on SGD and show that these models are not robust and limited to only certain types of slots. 
        \item We describe how to construct new datasets that teach models how to handle each of the slot types and conversation scenarios that are described above. 
        \item We train and evaluate models on SGD + our data and show that even small models having around 7-13B parameters can achieve accuracy comparable to or better than very large and capable models such as ChatGPT and PaLM. 
    \end{itemize}
\end{itemize}


==> sections/problem_definition.tex <==
\section{Problem Definition}
\label{sec:prob-def}

\begin{itemize}
    \item Given: conversation between a user and the system/agent up to turn $t$ $\mathcal{C}_t = [U_1, A_1, U_2, A_2, ..., U_t]$. $U_i$ is the user utterance and $A_i$ is the system/agent utterance.
    \item Given: a set of slots $\mathcal{S} = \{S_1, S_2, S_J\}$. Each $S_i \in S$ is a unique alphanumeric identifier of the slot. 
    \item Given: Natural language description of each slot. $\mathcal{D} = \{D_1, D_2, ..., D_J\}$. Where $D_i$ is the natural language description of the slot $S_i$
    \item Define $\mathcal{B}_t = \{(S_1, V_1^t), (S_2, V_2^t), ..., (S_J, V_J^t)\}$. $V_i^t$ is the value of slot $S_i$ inferred based on the conversation $\mathcal{C}_t$. Note that $V_i^t$ and $V_i^{(t+1)}$ may be different as the user might correct/update the information in the utterance $U_{(t+1)}$.
    \item The task is to learn the following function: $\mathcal{F}: (\mathcal{C}_t, \mathcal{S}, \mathcal{D}) \rightarrow \mathcal{B}_t$.
    \item Describe the metrics. Which ones do we use? Other papers use Joint Goal Accuracy.
\end{itemize}
